The Montreal Open Clusters and Associations (MOCA) Database: A Census of Nearby Associations, Open Clusters, and Young Substellar Objects within 500 pc of the Sun

We present the Montreal Open Clusters and Associations database (MOCAdb), a public MySQL database with a Python interface. MOCAdb provides a census of memberships for 10259 associations and open clusters, with a comprehensive compilation of literature measurements such as spectral types, kinematics, rotation periods, activity indices, spectral indices, and photometry. All known substellar objects are cataloged in MOCAdb, along with 2943 public spectra, to enable the characterization of substellar association members. MOCAdb also features periodically updated calculations such as Galactic UVW space velocities. We use this compilation to construct mappings between independent association definitions, and to update the BANYAN $\Sigma$ membership classification tool, which now includes 8125 associations. The BANYAN $\Sigma$ model construction is improved to account for heterogeneous and correlated errors and to capture complex association shapes using Gaussian mixture models. Combined with Gaia DR3, this enabled us to identify 11535 yet unrecognized candidate members of young associations within 500 pc, mostly M dwarfs. Our results corroborate a recent observation that systematics up to $\approx$4 km/s remain in Gaia DR3 radial velocities for A-type stars. We present an updated census of age-calibrated exoplanets and substellar objects: 134 age-calibrated exoplanet systems (plus 121 TESS exoplanet candidates), 99 of which did not appear to have known memberships so far, and 455 substellar (L0 or later) candidate members of young associations, 196 of which appear newly recognized. We bring the total of candidate isolated planetary-mass objects to 101, 53 of which are newly recognized candidate members.

==> tables/exoplanets.tex <==
\clearpage
\pagebreak
\begin{deluxetable*}{lcclcccc}
\tablewidth{0.985\textwidth}
\tablecaption{Age-calibrated exoplanets currently known.\label{tab:exoplanets}}
\tablehead{
\noalign{\vskip 1.0ex}
\colhead{\shortstack{Host Star\\ Designation}} & \colhead{$N_{\rm exo}$} & \colhead{Method} & \colhead{\texttt{moca\_aid}} & \colhead{\shortstack{Banyan~$\Sigma$\\ Prob. (\%)}} & \colhead{\shortstack{Mem.\\Ref.}} & \colhead{\shortstack{Age\\ (Myr)}} & \colhead{\shortstack{Age\\Ref.}}
}
\startdata
GJ 393 & 1 & RV & ABDMG & 99.3 & 1 & 133$^{+15}_{-20}$ & 2 \\
GJ 849 & 2 & RV & CRIUS197 & 94.8 & 3 & $\cdots$ & -- \\
HD 147513 & 1 & RV & CRIUS135 & 95.2 & 3 & 100-700 & 4 \\
GJ 163 & 3 & RV & HSC1711 & 85.1 & 3 & 260 (-190,+670) & 5 \\
GJ 3021 & 1 & RV & CRIUS203 & 97.3 & 3 & 670.0 +376.7/-241.1 & -- \\
LSPM J2116+0234 & 1 & RV & CARN & 92.7 & 3 & 200 & 6 \\
bet Pic & 2 & RV & BPMG & 99.0 & 7 & 26 $\pm$ 3 & 8 \\
GJ 9714 & 1 & RV & VELA & 91.7 & 3 & 2-9960 & -- \\
HD 114783 & 2 & RV & OCTN & 89.8 & 3 & 30-100 & 9 \\
HIP 12961 & 1 & RV & CRIUS197 & 98.7 & 3 & $\cdots$ & -- \\
HD 179949 & 1 & RV & VELA & 85.2 & 3 & 2-9960 & -- \\
HD 142415 & 1 & RV & CRIUS209 & 81.0 & 3 & $\cdots$ & -- \\
HS Psc & 1 & RV & ABDMG & 99.4 & 10 & 133$^{+15}_{-20}$ & 2 \\
30 Ari B & 1 & RV & CRIUS203 & 83.2 & 3 & 670.0 +376.7/-241.1 & -- \\
eps Tau & 1 & RV & HYA & 99.9 & 11 & 695$^{+85}_{-67}$ & 12 \\
HD 285507 & 1 & RV & HYA & 99.9 & 11 & 695$^{+85}_{-67}$ & 12 \\
HD 212301 & 1 & RV & MEL5 & 93.6 & 13 & 210 $\pm$ 27 & 14 \\
HD 135625 & 1 & RV & CRIUS209 & 97.4 & 3 & $\cdots$ & -- \\
HD 114082 & 1 & RV & GRSCOS27C & 99.5 & 3 & 14.6 & 15 \\
TAP 26 & 1 & RV & OH29 & 99.9 & 16 & 29.3 $\pm$ 1 & 17 \\
V830 Tau & 1 & RV & L1529 & 99.9 & 18 & 3.4 & 15 \\
CI Tau & 1 & RV & TAUMGLIU4 & 99.9 & 16 & 2.0 & 16 \\
Pr0201 & 1 & RV & PRA & 99.9 & 19 & 617 & 20 \\
Pr0211 & 2 & RV & CPRA & 99.9 & 21 & 617.0 & 20 \\
NGC 2682 Sand 364 & 1 & RV & NGC2682 & 99.7 & 22 & ~4000 & 22 \\
NGC 2682 YBP 401 & 1 & RV & NGC2682 & 99.9 & 22 & ~4000 & 22 \\
NGC 2682 Sand 978 & 1 & RV & NGC2682 & 99.9 & 22 & ~4000 & 22 \\
NGC 2682 Sand 1429 & 1 & RV & NGC2682 & 99.9 & 22 & ~4000 & 22 \\
NGC 2682 YBP 1194 & 1 & RV & NGC2682 & 99.8 & 22 & ~4000 & 22 \\
NGC 2682 YBP 1514 & 1 & RV & NGC2682 & 99.9 & 22 & ~4000 & 22 \\
IC 4651 9122 & 1 & RV & IC4651 & 99.9 & 22 & 1659.6 & 22 \\
BD-13 2130 & 1 & RV & NGC2423 & 99.9 & 22 & 1122.0 & 22 \\
AU Mic & 4 & T & BPMG & 98.1 & 7 & 26 $\pm$ 3 & 8 \\
TOI-431 & 3 & T & CRIUS197 & 93.0 & 3 & $\cdots$ & -- \\
TOI-2459 & 1 & T & MEL5 & 97.2 & 13 & 210 $\pm$ 27 & 14 \\
TOI-1224 & 2 & T & MEL5 & 99.8 & 13 & 210 $\pm$ 27 & 14 \\
TOI-2076 & 4 & T & CRIUS224 & 99.5 & 4 & $\cdots$ & -- \\
TOI-1807 & 1 & T & CRIUS224 & 99.6 & 4 & $\cdots$ & -- \\
TOI-5082 & 1 & T & CRIUS197 & 92.3 & 3 & $\cdots$ & -- \\
TOI-4364 & 1 & T & CHYA & 99.9 & 21 & 695$^{+85}_{-67}$ & 12 \\
K2-25 & 1 & T & HYA & 99.9 & 23 & 695$^{+85}_{-67}$ & 12 \\
HIP 94235 & 1 & T & ABDMG & 96.6 & 24 & 133$^{+15}_{-20}$ & 2 \\
K2-136 & 3 & T & HYA & 99.9 & 25 & 695$^{+85}_{-67}$ & 12 \\
TOI-3353 & 1 & T & ABDMG & 99.3 & 3 & 133$^{+15}_{-20}$ & 2 \\
HD 109833 & 2 & T & MEL4 & 95.0 & 26 & 23-26 & -- \\
TOI-1227 & 1 & T & HSC2523 & 99.9 & 3 & 7.0$^{+-4.2}_{-+4.1}$ & 5 \\
TOI-251 & 1 & T & SUN1 & 99.6 & 27 & 204 $\pm$ 45 & 28 \\
V1298 Tau & 4 & T & OH29 & 99.9 & 29 & 29.3 $\pm$ 1 & 17 \\
TOI-2048 & 1 & T & GRX & 85.5 & 30 & 300 $\pm$ 60 & 31 \\
TOI-451 & 3 & T & HSC1923 & 99.8 & 5 & 85 (-47,+69) & 5 \\
HIP 67522 & 2 & T & GRSCOS24 & 99.2 & 3 & 20.8 & 15 \\
KELT-20 & 1 & T & COH59 & 94.5 & 3 & 162.2 & 32 \\
K2-33 & 1 & T & GRSCOS17E & 99.9 & 15 & 7.2 & 15 \\
TOI-837 & 1 & T & IC2602 & 99.9 & 33 & 40.0$^{+1.9}_{-1.4}$ & 17 \\
TOI-6109 & 2 & T & APER & 99.9 & 34 & 79 +1.5/-2.3 & 12 \\
Kepler-411 & 4 & T & THEIA1275 & 99.7 & 35 & 794.3 & 32 \\
IRAS 04125+2902 & 1 & T & B209N & 99.9 & 18 & ~1 & -- \\
K2-264 & 2 & T & PRA & 99.9 & 36 & 617 & 20 \\
K2-95 & 1 & T & CPRA & 99.9 & 21 & 617.0 & 20 \\
K2-100 & 1 & T & CPRA & 99.9 & 21 & 617.0 & 20 \\
K2-101 & 1 & T & CPRA & 99.9 & 21 & 617.0 & 20 \\
K2-102 & 1 & T & CPRA & 99.9 & 21 & 617.0 & 20 \\
EPIC 211822797 & 1 & T & PRA & 99.9 & 37 & 617 & 20 \\
K2-104 & 1 & T & PRA & 99.9 & 36 & 617 & 20 \\
XO-3 & 1 & T & THEIA433 & 80.3 & 3 & 346.7 & 32 \\
TIC 434398831 & 2 & T & TAUOR2 & 99.9 & 15 & 41.5 & 15 \\
TOI-1518 & 1 & T & THEIA685 & 97.7 & 35 & 331.1 & 32 \\
KOI-7913 A & 1 & T & CEPHER & 93.8 & 3 & 11-710 & -- \\
Kepler-1930 & 1 & T & THEIA437 & 99.7 & 35 & 195.0 & 32 \\
Kepler-211 & 2 & T & MEL3 & 83.9 & 38 & 48-203 & -- \\
K2-231 & 1 & T & RUP147 & 99.9 & 39 & 3090.3 & 40 \\
Kepler-1928 & 1 & T & HSC572 & 99.9 & 5 & 103 (-55,+100) & 5 \\
Kepler-970 & 1 & T & MEL3 & 98.6 & 38 & 48-203 & -- \\
Kepler-1627 & 1 & T & CEPHER & 99.7 & 41 & 11-710 & -- \\
Kepler-1643 & 1 & T & RSG5 & 90.8 & 3 & 36.3 & 40 \\
TOI-1937 A & 1 & T & CNGC2516 & 82.4 & 3 & 195 $\pm$ 25 & 42 \\
NGTS-33 & 1 & T & THEIA97 & 96.2 & 3 & 32.4 & 32 \\
Kepler-326 & 3 & T & THEIA1194 & 89.8 & 3 & 524.8 & 32 \\
Kepler-67 & 1 & T & NGC6811 & 98.4 & 39 & 1100 $\pm$ 200 & 43 \\
Kepler-66 & 1 & T & NGC6811 & 98.3 & 39 & 1100 $\pm$ 200 & 43 \\
Kepler-1915 & 1 & T & NGC6866 & 98.9 & 5 & 645.7 & 22 \\
GJ 900 A & 1 & I & CRIUS203 & 98.7 & 4 & 670.0 +376.7/-241.1 & -- \\
G 196-3 & 1 & I & HSC517 & 98.8 & 3 & 162 $\pm$ 30 & -- \\
AF Lep & 1 & I & BPMG & 99.4 & 7 & 26 $\pm$ 3 & 8 \\
51 Eri & 1 & I & BPMG & 95.3 & 7 & 26 $\pm$ 3 & 8 \\
2MASS J01225093-2439505 & 1 & I & ABDMG & 91.4 & 44 & 133$^{+15}_{-20}$ & 2 \\
2MASS J02192210-3925225 & 1 & I & COL & 96.9 & 3 & 33.7$^{+2.0}_{-1.9}$ & 17 \\
HIP 99770 & 1 & I & ARG & 99.4 & 45 & 45-50 & 46 \\
HIP 21152 & 1 & I & HYA & 99.9 & 11 & 695$^{+85}_{-67}$ & 12 \\
PZ Tel & 1 & I & BPMG & 99.1 & 7 & 26 $\pm$ 3 & 8 \\
GU Psc & 1 & I & ABDMG & 99.7 & 47 & 133$^{+15}_{-20}$ & 2 \\
AB Pic & 1 & I & CAR & 99.9 & 48 & 33.7$^{+2.0}_{-1.9}$ & 17 \\
kap And & 1 & I & HSC517 & 81.6 & 3 & 162 $\pm$ 30 & -- \\
2MASS J12073346-3932539 & 1 & I & TWA & 99.9 & 3 & 10 & 49 \\
HD 95086 & 1 & I & MEL4 & 99.0 & 26 & 23-26 & -- \\
TYC 8998-760-1 & 2 & I & MEL4 & 99.9 & 26 & 23-26 & -- \\
2MASS J11550485-7919108 & 1 & I & HSC2515 & 99.9 & 5 & 120 (-100,+460) & 5 \\
HD 106906 & 1 & I & HSC2468 & 99.9 & 3 & 8.4 $\pm$ 4.0 & 5 \\
b Cen A & 1 & I & RATZSCO20 & 98.9 & 50 & 15.2 (-0.3,+0.9) & 51 \\
HIP 65426 & 1 & I & GRSCOS26 & 99.3 & 3 & 21.7 & 15 \\
HD 100546 & 1 & I & EPSC & 99.6 & 3 & 3.7 & 52 \\
GSC 06214-00210 & 1 & I & CWNU1143 & 99.8 & 3 & 18.5 (-8.3,+15.0) & 5 \\
YSES 2 & 1 & I & MEL4 & 99.2 & 26 & 23-26 & -- \\
PDS 70 & 2 & I & RATZSCO20 & 99.2 & 50 & 15.2 (-0.3,+0.9) & 51 \\
HD 284149 A & 1 & I & OH29 & 99.9 & 29 & 29.3 $\pm$ 1 & 17 \\
2MASS J04414489+2301513 & 1 & I & L1529 & 99.8 & 18 & 3.4 & 15 \\
2MASS J03590986+2009361 & 1 & I & OH29 & 99.9 & 3 & 29.3 $\pm$ 1 & 17 \\
FU Tau & 1 & I & L1529 & 99.9 & 18 & 3.4 & 15 \\
2MASS J04372171+2651014 & 1 & I & HD28354 & 99.0 & 18 & 6.0$^{+4.5}_{-2.6}$ & 18 \\
Oph 11 & 1 & I & GRSCOS17A & 99.7 & 3 & 16.2 & 15 \\
DH Tau & 1 & I & L1529 & 99.9 & 3 & 3.4 & 15 \\
WISPIT 2 & 1 & I & SCYA78 & 92.5 & 41 & 18 & 41 \\
HIP 78530 & 1 & I & OCSN96 & 98.9 & 3 & 4.7 $\pm$ 1.5 & 5 \\
HD 135344 A & 1 & I & GRSCOS19 & 96.0 & 3 & 15.3 & 15 \\
USco1621 A & 1 & I & ROPH & 98.6 & 53 & < 2 & 54 \\
HD 143811 A & 1 & I & RATZSCO14 & 94.9 & 3 & 14.8 $\pm$ 0.7 & 51 \\
CFHTWIR-Oph 98 A & 1 & I & HSC2919 & 99.9 & 3 & 27 (-17,+57) & 5 \\
1RXS J160929.1-210524 & 1 & I & OCSN96 & 99.8 & 5 & 4.7 $\pm$ 1.5 & 5 \\
ROXs 12 & 1 & I & HSC2919 & 99.8 & 5 & 27 (-17,+57) & 5 \\
ITG 15 A & 1 & I & L1527 & 99.9 & 18 & 0.6$^{+1.1}_{-0.4}$ & 18 \\
USco CTIO 108 & 1 & I & OCSN98 & 99.7 & 3 & 4.5 (-1.8,+1.2) & 5 \\
HIP 81208 C & 1 & I & SCOBODY & 99.9 & 3 & 12-20 & -- \\
ROXs 42 B & 1 & I & ROPH & 98.6 & 55 & < 2 & 54 \\
HIP 77900 & 1 & I & GRSCOS17H & 97.0 & 3 & 10.2 & 15 \\
GQ Lup & 1 & I & LUPI & 99.7 & 56 & 5.9 & 15 \\
HIP 79098 AB & 1 & I & GRSCOS17H & 98.5 & 3 & 10.2 & 15 \\
MWC 758 & 1 & I & GRTAUS9B & 99.9 & 15 & 11.5 & 15 \\
AB Aur & 1 & I & TAUMGLIU8 & 99.4 & 16 & 4.0 & 16 \\
LkCa 15 & 2 & I & TAUMGLIU4 & 99.9 & 16 & 2.0 & 16 \\
2MASS J11011926-7732383 & 1 & I & CHAI & 99.6 & 5 & 4.6 & 15 \\
CT Cha & 1 & I & CHAI & 99.8 & 57 & 4.6 & 15 \\
CHXR 73 & 1 & I & CHAI & 99.7 & 58 & 4.6 & 15 \\
OGLE-2013-BLG-0132L & 1 & Microlensing & THEIA1007 & 99.0 & 3 & 512.9 & 32 \\
OGLE-2016-BLG-1067L & 1 & Microlensing & THEIA1112 & 98.3 & 3 & 309.0 & 32 \\
\enddata
\tablerefs{(1)~\cite{2009AA...508..833D}, (2)~\cite{2018ApJ...861L..13G}, (3)~This Paper, (4)~\cite{2022ApJ...939...94M}, (5)~\cite{2023AA...673A.114H}, (6)~\cite{2006ApJ...649L.115Z}, (7)~\cite{2001ApJ...562L..87Z}, (8)~\cite{2014ApJ...792...37M}, (9)~\cite{2013ApJ...778....5Z}, (10)~\cite{2010AJ....140..119S}, (11)~\cite{1998AA...331...81P}, (12)~\cite{2022AA...664A..70G}, (13)~\cite{2024arXiv240605234T}, (14)~\cite{2024AJ....168...41T}, (15)~\cite{2021ApJ...917...23K}, (16)~\cite{2021ApJS..254...20L}, (17)~\cite{2024AJ....167...19L}, (18)~\cite{2023AJ....165...37L}, (19)~\cite{2014ApJ...795..161D}, (20)~\cite{2018ApJ...863...67G}, (21)~\cite{2019AA...627A...4R}, (22)~\cite{2021AA...647A..19T}, (23)~\cite{2018ApJ...862..138G}, (24)~\cite{2010AA...520A..15M}, (25)~\cite{2019AA...621L...3M}, (26)~\cite{2023AJ....165...85W}, (27)~\cite{2023arXiv230503255S}, (28)~\cite{2023ApJ...952...68S}, (29)~\cite{2017AJ....153..257O}, (30)~\cite{2019ApJ...877...12T}, (31)~\cite{2022AA...657L...3M}, (32)~\cite{2020AJ....160..279K}, (33)~\cite{2019AA...623A.112D}, (34)~\cite{2021AA...645A..84M}, (35)~\cite{2019AJ....158..122K}, (36)~\cite{2019MNRAS.486.5405G}, (37)~\cite{2007AJ....134.2340K}, (38)~\cite{2022AJ....164...88B}, (39)~\cite{2020ApJ...904..140C}, (40)~\cite{2020AA...640A...1C}, (41)~\cite{2023ApJ...954..134K}, (42)~\cite{2018AJ....156..165C}, (43)~\cite{2011AJ....141...92J}, (44)~\cite{2014ApJ...788...81M}, (45)~\cite{2011ApJ...732...61Z}, (46)~\cite{2019ApJ...870...27Z}, (47)~\cite{2012AJ....143...80S}, (48)~\cite{2003ApJ...599..342S}, (49)~\cite{2015MNRAS.454..593B}, (50)~\cite{2023AA...677A..59R}, (51)~\cite{2023AA...678A..71R}, (52)~\cite{2013MNRAS.435.1325M}, (53)~\cite{2019AA...626A..80C}, (54)~\cite{2008hsf2.book..351W}, (55)~\cite{2015ApJ...813...83C}, (56)~\cite{2020AJ....160..186L}, (57)~\cite{2003AA...404..913S}, (58)~\cite{2004ApJ...602..816L}.}
\end{deluxetable*}


==> tables/exoplanets_candidates.tex <==
\clearpage
\pagebreak
\begin{deluxetable*}{lcccccc}
\tablewidth{0.985\textwidth}
\tablecaption{Age-calibrated TESS exoplanets candidates.\label{tab:exoplanet_candidates}}
\tablehead{
\noalign{\vskip 1.0ex}
\colhead{\shortstack{Host Star\\ Designation}} & \colhead{$N_{\rm exo}$} & \colhead{\texttt{moca\_aid}} & \colhead{\shortstack{Banyan~$\Sigma$\\ Prob. (\%)}} & \colhead{\shortstack{Mem.\\Ref.}} & \colhead{\shortstack{Age\\ (Myr)}} & \colhead{\shortstack{Age\\Ref.}}
}
\startdata
TIC 141141249 & 1 & ARG & 93.1 & 1 & 45-50 & 2 \\
TIC 278198753 & 1 & CAR & 81.3 & 1 & 33.7$^{+2.0}_{-1.9}$ & 3 \\
TIC 325468685 & 1 & CRIUS131 & 82.5 & 1 & 569.1 +619.1/-239.3 & -- \\
TIC 441420236 & 1 & BPMG & 98.1 & 4 & 26 $\pm$ 3 & 5 \\
TIC 31374837 & 1 & CRIUS197 & 93.0 & 1 & $\cdots$ & -- \\
TIC 192790476 & 1 & MEL5 & 97.2 & 6 & 210 $\pm$ 27 & 7 \\
TIC 299798795 & 1 & MEL5 & 99.8 & 6 & 210 $\pm$ 27 & 7 \\
TIC 51024887 & 1 & OCEMG & 90.1 & 1 & ~500-600 & 8 \\
TIC 27491137 & 1 & CRIUS224 & 99.5 & 9 & $\cdots$ & -- \\
TIC 180695581 & 1 & CRIUS224 & 99.6 & 9 & $\cdots$ & -- \\
TIC 437011608 & 1 & CRIUS197 & 92.3 & 1 & $\cdots$ & -- \\
TIC 4070275 & 1 & CHYA & 99.9 & 10 & 695$^{+85}_{-67}$ & 11 \\
TIC 434226736 & 1 & HYA & 99.9 & 12 & 695$^{+85}_{-67}$ & 11 \\
TIC 244161191 & 1 & COL & 92.7 & 1 & 33.7$^{+2.0}_{-1.9}$ & 3 \\
TIC 20182165 & 1 & OCTN & 97.5 & 13 & 30-100 & 13 \\
TIC 77951245 & 1 & COL & 99.9 & 12 & 33.7$^{+2.0}_{-1.9}$ & 3 \\
TIC 419957393 & 1 & OCTN & 96.3 & 1 & 30-100 & 13 \\
TIC 464646604 & 1 & ABDMG & 96.6 & 14 & 133$^{+15}_{-20}$ & 15 \\
TIC 18310799 & 1 & HYA & 99.9 & 16 & 695$^{+85}_{-67}$ & 11 \\
TIC 311183180 & 1 & CHYA & 86.5 & 1 & 695$^{+85}_{-67}$ & 11 \\
TIC 298981199 & 1 & OCTN & 99.2 & 1 & 30-100 & 13 \\
TIC 311271011 & 1 & CRIUS223 & 99.4 & 9 & 100-700 & -- \\
TIC 93125144 & 1 & ABDMG & 82.9 & 14 & 133$^{+15}_{-20}$ & 15 \\
TIC 39200363 & 1 & CRIUS205 & 99.9 & 9 & $\cdots$ & -- \\
TIC 391903064 & 1 & ABDMG & 99.3 & 1 & 133$^{+15}_{-20}$ & 15 \\
TIC 360630575 & 1 & MEL4 & 95.0 & 17 & 23-26 & -- \\
TIC 157081737 & 1 & THEIA301 & 97.9 & 18 & 195.0 & 19 \\
TIC 360156606 & 1 & HSC2523 & 99.9 & 1 & 7.0$^{+-4.2}_{-+4.1}$ & 20 \\
TIC 224225541 & 1 & SUN1 & 99.6 & 21 & 204 $\pm$ 45 & 22 \\
TIC 166053959 & 1 & GRX & 88.0 & 23 & 300 $\pm$ 60 & 24 \\
TIC 359357695 & 1 & HSC2523 & 99.9 & 1 & 7.0$^{+-4.2}_{-+4.1}$ & 20 \\
TIC 142938659 & 1 & XFOR & 99.9 & 25 & 33.7$^{+2.0}_{-1.9}$ & 3 \\
TIC 159873822 & 1 & GRX & 85.5 & 23 & 300 $\pm$ 60 & 24 \\
TIC 257605131 & 1 & HSC1923 & 99.8 & 20 & 85 (-47,+69) & 20 \\
TIC 14091633 & 1 & OCT & 99.7 & 26 & 30-40 & 27 \\
TIC 135036669 & 1 & FCCN & 99.9 & 28 & 29.2 $\pm$ 4.5 & 29 \\
TIC 69679391 & 1 & COH59 & 94.5 & 1 & 162.2 & 19 \\
TIC 405484221 & 1 & PLE & 99.7 & 30 & 127.4 +6.3/-10 & 11 \\
TIC 460205581 & 1 & IC2602 & 99.9 & 31 & 40.0$^{+1.9}_{-1.4}$ & 3 \\
TIC 384984325 & 1 & APER & 99.9 & 32 & 79 +1.5/-2.3 & 11 \\
TIC 130415266 & 1 & HSC1964 & 90.8 & 20 & 88 (-44,+64) & 20 \\
TIC 229944666 & 1 & CRIUS158 & 98.7 & 9 & $\cdots$ & -- \\
TIC 459952217 & 1 & MUTAU & 90.6 & 33 & 61 & 33 \\
TIC 399954349 & 1 & THEIA1275 & 99.7 & 18 & 794.3 & 19 \\
TIC 219205407 & 1 & VELA & 81.6 & 34 & 2-9960 & -- \\
TIC 457939414 & 1 & THAN & 99.9 & 1 & 37-55 & -- \\
TIC 367855829 & 1 & CRIUS158 & 84.7 & 1 & $\cdots$ & -- \\
TIC 96246348 & 1 & CWNU1013 & 97.8 & 1 & 400 (-330,+2500) & 20 \\
TIC 313506357 & 1 & THEIA1275 & 91.5 & 1 & 794.3 & 19 \\
TIC 66620917 & 1 & CPL10 & 94.3 & 1 & 110 $\pm$ 20 & 35 \\
TIC 276250096 & 1 & THEIA1275 & 87.0 & 1 & 794.3 & 19 \\
TIC 316916655 & 1 & CWNU1018 & 99.7 & 20 & 153 (-74,+110) & 20 \\
TIC 307733361 & 1 & CPRA & 99.9 & 10 & 617.0 & 36 \\
TIC 184892124 & 1 & PRA & 99.9 & 37 & 617 & 36 \\
TIC 300011941 & 1 & VCG4S2 & 97.9 & 1 & 37.8 & 34 \\
TIC 160328683 & 1 & OCT & 94.1 & 1 & 30-40 & 27 \\
TIC 363761216 & 1 & THEIA685 & 93.5 & 1 & 331.1 & 19 \\
TIC 32498058 & 1 & CRIUS188 & 99.5 & 1 & $\cdots$ & -- \\
TIC 8400842 & 1 & THEIA433 & 80.3 & 1 & 346.7 & 19 \\
TIC 129991079 & 1 & UPK303 & 99.7 & 20 & 81.3 & 35 \\
TIC 151284882 & 1 & HSC1553 & 99.9 & 20 & 53 $\pm$ 11 & 38 \\
TIC 148479278 & 1 & VCG4S2 & 99.9 & 1 & 37.8 & 34 \\
TIC 222485202 & 1 & THEIA1356 & 91.2 & 1 & 724.4 & 19 \\
TIC 427761355 & 1 & THEIA685 & 97.7 & 18 & 331.1 & 19 \\
TIC 143994283 & 1 & THEIA1185 & 95.4 & 1 & 631.0 & 19 \\
TIC 456305193 & 1 & CRSG2 & 95.5 & 1 & 126 & 39 \\
TIC 270238522 & 1 & THEIA685 & 81.4 & 1 & 331.1 & 19 \\
TIC 90544017 & 1 & VELA & 98.4 & 1 & 2-9960 & -- \\
TIC 363260203 & 1 & HSC2462 & 80.2 & 1 & 40 (-20,+28) & 20 \\
TIC 59859387 & 1 & ALES3 & 99.9 & 40 & 631.0 & 35 \\
TIC 94727308 & 1 & PERSS2B & 99.8 & 34 & 17.1 & 34 \\
TIC 123898871 & 1 & VELA & 99.6 & 18 & 2-9960 & -- \\
TIC 268914377 & 1 & VCG4S5 & 99.8 & 1 & 32.1 & 34 \\
TIC 149990841 & 1 & SCYA10 & 97.1 & 1 & 27 & 41 \\
TIC 4294779 & 1 & GRORIS1B & 99.9 & 1 & 20.0 & 34 \\
TIC 81419525 & 1 & GVEL1 & 99.9 & 1 & 5.5 $\pm$ 1.0 & 42 \\
TIC 13419950 & 1 & ROSL6 & 92.4 & 1 & 91.2 & 35 \\
TIC 131743355 & 1 & VCG4S5 & 98.0 & 1 & 32.1 & 34 \\
TIC 400595342 & 1 & HSC2196 & 99.9 & 20 & 190 (-100,+230) & 20 \\
TIC 15247229 & 1 & ROSL6 & 99.9 & 25 & 91.2 & 35 \\
TIC 237185205 & 1 & STEP1 & 99.9 & 20 & 28.8 & 35 \\
TIC 340458804 & 1 & UPK540 & 99.9 & 20 & 38.0 & 35 \\
TIC 340559155 & 1 & VELA & 83.5 & 1 & 2-9960 & -- \\
TIC 349966879 & 1 & NGC2516 & 99.5 & 1 & 195 $\pm$ 25 & 43 \\
TIC 207277638 & 1 & HSC1634 & 96.1 & 1 & 110 (-66,+160) & 20 \\
TIC 410450228 & 1 & NGC2516 & 99.9 & 32 & 195 $\pm$ 25 & 43 \\
TIC 147430118 & 1 & VELA & 88.9 & 1 & 2-9960 & -- \\
TIC 308307606 & 1 & NGC2516 & 99.5 & 44 & 195 $\pm$ 25 & 43 \\
TIC 268301217 & 1 & CNGC2516 & 82.4 & 1 & 195 $\pm$ 25 & 43 \\
TIC 89617284 & 1 & CNGC2516 & 92.7 & 1 & 195 $\pm$ 25 & 43 \\
TIC 371673488 & 1 & RSG7 & 97.1 & 25 & 39.8 & 35 \\
TIC 80275202 & 1 & VCG7 & 97.9 & 1 & 14.4 & 34 \\
TIC 180987952 & 1 & TRU10 & 94.9 & 20 & 33.1 & 35 \\
TIC 384549882 & 1 & CWNU1020 & 99.9 & 20 & 34 (-17,+23) & 20 \\
TIC 308425348 & 1 & NGC3532 & 99.6 & 45 & 360 $\pm$ 20 & 43 \\
TIC 378613125 & 1 & HSC2376 & 99.9 & 20 & 86 (-40,+69) & 20 \\
TIC 388934707 & 1 & THEIA6046 & 95.7 & 1 & 3800 (-1200,+4100) & 19 \\
TIC 154353849 & 1 & UPK168 & 93.6 & 1 & 37.2 & 40 \\
TIC 376682699 & 1 & UPK230 & 99.6 & 20 & 75.9 & 40 \\
TIC 395143000 & 1 & THEIA836 & 83.5 & 1 & 104 (-40,+74) & 19 \\
TIC 34466256 & 1 & THEIA6046 & 98.3 & 20 & 3800 (-1200,+4100) & 19 \\
TIC 420288086 & 1 & NGC225 & 99.9 & 20 & 93 (-34,+73) & 20 \\
TIC 89759617 & 1 & THEIA470 & 98.9 & 20 & 180 (-75,+140) & 19 \\
TIC 115451738 & 1 & UPK369 & 80.4 & 20 & 135 (-49,+92) & 20 \\
TIC 396368313 & 1 & UPK585 & 99.8 & 20 & 95 (-40,+60) & 20 \\
TIC 50120414 & 1 & HSC1103 & 99.1 & 20 & 63 (-28,+45) & 20 \\
TIC 108835813 & 1 & THEIA1147 & 92.8 & 19 & 660 (-290,+390) & 19 \\
TIC 27476314 & 1 & HSC1471 & 90.5 & 1 & 47 (-21,+47) & 20 \\
TIC 443115574 & 1 & NGC2215 & 99.7 & 20 & 707.9 & 40 \\
TIC 16264917 & 1 & HSC2777 & 93.2 & 1 & 18.0 (-6.8,+17.0) & 20 \\
TIC 462162963 & 1 & NGC3114 & 99.3 & 20 & 144.5 & 40 \\
TIC 53047383 & 1 & THEIA1179 & 85.0 & 20 & 260 (-110,+160) & 19 \\
TIC 67031480 & 1 & HSC1350 & 99.4 & 20 & 52 (-20,+32) & 20 \\
TIC 172754786 & 1 & UBC582 & 99.9 & 20 & 8.5 (-3.1,+3.7) & 20 \\
TIC 195199644 & 1 & ROSL7 & 99.4 & 20 & 175 (-61,+100) & 20 \\
TIC 259165246 & 1 & CWNU110 & 85.6 & 1 & 217 (-92,+150) & 20 \\
TIC 187861378 & 1 & THEIA2299 & 99.9 & 20 & 220 (-100,+160) & 19 \\
TIC 388393034 & 1 & CASA20 & 99.9 & 20 & 350 (-140,+190) & 20 \\
TIC 76545118 & 1 & TAUOR4 & 99.7 & 1 & 21.3 & 34 \\
TIC 304426002 & 1 & HSC2474 & 99.7 & 1 & 1280 (-580,+1600) & 20 \\
TIC 144970275 & 1 & ESO430_18 & 93.7 & 20 & 85 (-36,+54) & 20 \\
\enddata
\tablerefs{(1)~This Paper, (2)~\cite{2019ApJ...870...27Z}, (3)~\cite{2024AJ....167...19L}, (4)~\cite{2001ApJ...562L..87Z}, (5)~\cite{2014ApJ...792...37M}, (6)~\cite{2024arXiv240605234T}, (7)~\cite{2024AJ....168...41T}, (8)~\cite{2022arXiv220800070G}, (9)~\cite{2022ApJ...939...94M}, (10)~\cite{2019AA...627A...4R}, (11)~\cite{2022AA...664A..70G}, (12)~\cite{2018ApJ...862..138G}, (13)~\cite{2013ApJ...778....5Z}, (14)~\cite{2010AA...520A..15M}, (15)~\cite{2018ApJ...861L..13G}, (16)~\cite{2019AA...621L...3M}, (17)~\cite{2023AJ....165...85W}, (18)~\cite{2019AJ....158..122K}, (19)~\cite{2020AJ....160..279K}, (20)~\cite{2023AA...673A.114H}, (21)~\cite{2023arXiv230503255S}, (22)~\cite{2023ApJ...952...68S}, (23)~\cite{2019ApJ...877...12T}, (24)~\cite{2022AA...657L...3M}, (25)~\cite{2018AA...618A..93C}, (26)~\cite{2018ApJ...860...43G}, (27)~\cite{2015MNRAS.447.1267M}, (28)~\cite{2024AJ....168..159L}, (29)~\cite{2022ApJ...941..143K}, (30)~\cite{2007ApJS..172..663S}, (31)~\cite{2019AA...623A.112D}, (32)~\cite{2021AA...645A..84M}, (33)~\cite{2020ApJ...903...96G}, (34)~\cite{2021ApJ...917...23K}, (35)~\cite{2020AA...640A...1C}, (36)~\cite{2018ApJ...863...67G}, (37)~\cite{2019MNRAS.486.5405G}, (38)~\cite{2023AJ....165...37L}, (39)~\cite{2016AA...595A..22R}, (40)~\cite{2021AA...647A..19T}, (41)~\cite{2023ApJ...954..134K}, (42)~\cite{2009MNRAS.400L..20E}, (43)~\cite{2018AJ....156..165C}, (44)~\cite{2008AJ....136..118F}, (45)~\cite{2018AA...616A..10G}.}
\end{deluxetable*}


==> tables/missions_preview.tex <==
\clearpage
\pagebreak
\begin{deluxetable*}{llc}
\tablewidth{0.985\textwidth}
\tablecaption{External Catalogs Cross-Matched with MOCAdb Entries.\label{tab:missions}}
\tablehead{
\noalign{\vskip 1.0ex}
\colhead{\shortstack{MOCAdb\\ Table}} & \colhead{\shortstack{Mission\\ Name}} & \colhead{Reference}
}
\startdata
\texttt{cat\_2mass} & 2MASS PSC & 1 \\
\texttt{cat\_apogeedr16\_allstars} & APOGEE DR16 & 2 \\
\texttt{cat\_decapsdr2} & DECAPS DR2 & 3 \\
\texttt{cat\_denisdr3} & DENIS DR3 & 4 \\
\texttt{cat\_desdr2} & DES DR2 & 5 \\
\texttt{cat\_gaiadr1} & Gaia DR1 & 6 \\
\texttt{cat\_gaiadr2} & Gaia DR2 & 7 \\
\texttt{cat\_gaiaedr3} & Gaia EDR3 & 8 \\
\texttt{cat\_gaiadr3} & Gaia DR3 & 9 \\
\texttt{cat\_galahdr3} & GALAH DR3 & 10 \\
\texttt{cat\_galex\_gr67} & Galex GR67 & 11 \\
\texttt{cat\_hipparcos} & Hipparcos 2007 reduction & 12 \\
\texttt{cat\_nscdr2} & NSC DR2 & 13 \\
\texttt{cat\_ps1dr2} & PS1 DR2 & 14 \\
\texttt{cat\_ravedr6} & RAVE DR6 & 15 \\
\texttt{cat\_rosat} & ROSAT All-Sky & 16 \\
\texttt{cat\_splusdr4} & S-PLUS DR4 & 17 \\
\texttt{cat\_sdssdr17} & SDSS DR17 & 18 \\
\texttt{cat\_smssdr4} & SMSS DR4 & 19 \\
\texttt{cat\_uhsdr3} & UHS DR3 & 20 \\
\texttt{cat\_ukidssdxsdr11plus} & UKIDSSDXS DR11PLUS & 21 \\
\texttt{cat\_ukidssgcsdr11plus} & UKIDSSGCS DR11PLUS & 21 \\
\texttt{cat\_ukidssgpsdr11plus} & UKIDSSGPS DR11PLUS & 21 \\
\texttt{cat\_ukidsslasdr11plus} & UKIDSSLAS DR11PLUS & 21 \\
\texttt{cat\_vhsdr6} & VHS DR6 & 22 \\
\texttt{cat\_videodr5} & VIDEO DR5 & 23 \\
\texttt{cat\_vikingdr4} & VIKING DR4 & 24 \\
\texttt{cat\_viracdr4\_plx} & VIRAC DR4 & 25 \\
\texttt{cat\_vmcdr5} & VMC DR5 & 26 \\
\texttt{cat\_vvvdr5} & VVV DR5 & 27 \\
\texttt{cat\_wise} & WISE All-Sky SC & 28 \\
\texttt{cat\_allwise} & WISE AllWISE & 29 \\
\texttt{cat\_catwise} & WISE CatWISE & 30 \\
\enddata
\tablerefs{(1)~\cite{2006AJ....131.1163S}, (2)~\cite{2020ApJS..249....3A}, (3)~\cite{2023ApJS..264...28S}, (4)~\cite{1994ApSS.217....3E}, (5)~\cite{2021ApJS..255...20A}, (6)~\cite{2016AA...595A...2G}, (7)~\cite{2018AA...616A...1G}, (8)~\cite{2021AA...649A...1G}, (9)~\cite{2023AA...674A...1G}, (10)~\cite{2025PASA...42...51B}, (11)~\cite{2017ApJS..230...24B}, (12)~\cite{2007AA...474..653V_DUP}, (13)~\cite{2021AJ....161..192N}, (14)~\cite{2016arXiv161205560C}, (15)~\cite{2020AJ....160...82S}, (16)~\cite{1999AA...349..389V}, (17)~\cite{2024AA...689A.249H}, (18)~\cite{2022ApJS..259...35A}, (19)~\cite{2024PASA...41...61O}, (20)~\cite{2025AJ....170...86S}, (21)~\cite{2007MNRAS.379.1599L}, (22)~\cite{2013Msngr.154...35M}, (23)~\cite{2022RNAAS...6..109H}, (24)~\cite{2013Msngr.154...32E}, (25)~\cite{2018MNRAS.474.1826S}, (26)~\cite{2011AA...527A.116C}, (27)~\cite{2012AA...537A.107S}, (28)~\cite{2010AJ....140.1868W}, (29)~\cite{2014ApJ...783..122K}, (30)~\cite{2021ApJS..253....8M}.}
\end{deluxetable*}


==> tables/mocadb_tables.tex <==
\begin{deluxetable*}{lcc}
\tablewidth{0.985\textwidth}
\tablecaption{List of Tables in MOCAdb.\label{tab:mocadb_tables}}
\tablehead{
\noalign{\vskip 1.0ex}
\colhead{Table Name} & \colhead{Number of Columns} & \colhead{Number of Rows}
}
\startdata
\texttt{moca\_associations} & 18 & 10261 \\
\texttt{moca\_changelog} & 11 & 61408 \\
\texttt{moca\_companions} & 17 & 36887 \\
\texttt{moca\_spectral\_indices} & 15 & 78 \\
\texttt{moca\_instruments} & 6 & 73 \\
\texttt{moca\_missions} & 21 & 42 \\
\texttt{moca\_banyan\_sigma\_models} & 16 & 1 \\
\texttt{moca\_objects} & 18 & 3234191 \\
\texttt{moca\_spectra\_packages} & 30 & 28 \\
\texttt{moca\_object\_properties} & 10 & 22 \\
\texttt{moca\_publications} & 19 & 5507 \\
\texttt{moca\_extinction\_by\_spectral\_reference} & 12 & 2093 \\
\texttt{moca\_spectral\_type\_references} & 16 & 161 \\
\texttt{moca\_sequences} & 35 & 7 \\
\texttt{moca\_chemical\_species} & 14 & 10 \\
\texttt{moca\_spectra} & 69 & 4064 \\
\texttt{moca\_photometry\_systems} & 18 & 109 \\
\texttt{moca\_object\_types} & 5 & 13 \\
\texttt{moca\_membership\_types} & 7 & 6 \\
\texttt{cat\_2mass} & 73 & 2152213 \\
\texttt{cat\_apogeedr16\_allstars} & 176 & 439475 \\
\texttt{cat\_apogeedr16\_allvisits} & 70 & 1679797 \\
\texttt{cat\_allwise} & 305 & 1371102 \\
\texttt{cat\_catwise} & 200 & 1769974 \\
\texttt{cat\_decapsdr2} & 223 & 2004 \\
\texttt{cat\_denisdr3} & 87 & 23366 \\
\texttt{cat\_desdr1} & 184 & 22169 \\
\texttt{cat\_desdr2} & 238 & 41963 \\
\texttt{cat\_erassdr1} & 256 & 833615 \\
\texttt{cat\_euclidq1} & 664 & 589 \\
\texttt{cat\_gaiadr1} & 66 & 145784 \\
\texttt{cat\_gaiadr2} & 103 & 3081410 \\
\texttt{cat\_gaiadr3} & 164 & 3064316 \\
\texttt{cat\_gaiaedr3} & 109 & 609388 \\
\texttt{cat\_galahdr3} & 191 & 6583 \\
\texttt{cat\_galex\_gr67} & 103 & 43920 \\
\texttt{cat\_hipparcos} & 33 & 118182 \\
\texttt{cat\_gaiadr3\_binary\_masses} & 19 & 10549 \\
\texttt{cat\_gaiadr3\_vari\_rotation\_modulation} & 72 & 16433 \\
\texttt{cat\_exoplanets\_nasa} & 295 & 5154 \\
\texttt{cat\_exoplanet\_candidates\_tess\_nasa} & 102 & 6286 \\
\texttt{cat\_nscdr2} & 113 & 114386 \\
\texttt{cat\_panstarrsdr1} & 141 & 167638 \\
\texttt{cat\_panstarrsdr2} & 142 & 160418 \\
\texttt{cat\_gaiadr3\_astrophysical\_parameters} & 232 & 2981549 \\
\texttt{cat\_viracdr4\_plx} & 37 & 6906 \\
\texttt{cat\_ps1dr2} & 310 & 91686 \\
\texttt{cat\_ravedr6} & 44 & 498927 \\
\texttt{cat\_rosat} & 18 & 12026 \\
\texttt{cat\_sdssdr17} & 525 & 4111 \\
\texttt{cat\_simbad} & 109 & 271889 \\
\texttt{cat\_smssdr4} & 134 & 7 \\
\texttt{cat\_splusdr4} & 379 & 10308 \\
\texttt{cat\_uhsdr2} & 91 & 27496 \\
\texttt{cat\_uhsdr3} & 129 & 59294 \\
\texttt{cat\_ukidssdxsdr11plus} & 125 & 208 \\
\texttt{cat\_ukidssgcsdr11plus} & 242 & 2579 \\
\texttt{cat\_ukidssgcsdr9} & 114 & 49592 \\
\texttt{cat\_ukidssgpsdr11plus} & 205 & 1955 \\
\texttt{cat\_ukidsslasdr11plus} & 226 & 8441 \\
\texttt{cat\_ukidsslasdr9} & 100 & 203920 \\
\texttt{cat\_ultracoolsheet} & 250 & 3525 \\
\texttt{cat\_vhsdr4} & 142 & 84368 \\
\texttt{cat\_vhsdr6} & 167 & 47949 \\
\texttt{cat\_videodr5} & 181 & 87 \\
\texttt{cat\_vikingdr4} & 191 & 3631 \\
\texttt{cat\_vmcdr5} & 123 & 411 \\
\texttt{cat\_vvvdr5} & 324 & 144 \\
\texttt{cat\_wise} & 293 & 50152 \\
\texttt{data\_association\_ages} & 32 & 60461 \\
\texttt{data\_object\_ages} & 29 & 731078 \\
\texttt{data\_photometric\_bandpasses} & 6 & 11766 \\
\texttt{data\_convective\_blueshift} & 32 & 8491537 \\
\texttt{data\_median\_colors} & 17 & 1048 \\
\texttt{data\_equatorial\_coordinates} & 51 & 17863120 \\
\texttt{data\_rejected\_membership\_spatial\_kinematic\_distances} & 18 & 21 \\
\texttt{data\_distances} & 38 & 7709048 \\
\texttt{data\_extinction} & 27 & 1146257 \\
\texttt{data\_xray\_flux} & 30 & 9697 \\
\texttt{data\_inclinations} & 37 & 4942 \\
\texttt{data\_spectral\_indices} & 34 & 8803258 \\
\texttt{data\_masses} & 35 & 8853348 \\
\texttt{data\_memberships} & 18 & 4415932 \\
\texttt{data\_rejected\_memberships} & 20 & 108 \\
\texttt{data\_association\_metallicities} & 28 & 151 \\
\texttt{data\_banyan\_sigma\_models} & 71 & 42 \\
\texttt{data\_proper\_motions} & 37 & 10855342 \\
\texttt{data\_parallaxes} & 32 & 6274692 \\
\texttt{data\_rejected\_membership\_parameters} & 13 & 124 \\
\texttt{data\_rotation\_periods} & 37 & 2189488 \\
\texttt{data\_photometry} & 53 & 26126912 \\
\texttt{data\_object\_properties} & 22 & 217624 \\
\texttt{data\_radii} & 32 & 7003852 \\
\texttt{data\_gravitational\_redshift} & 32 & 6279040 \\
\texttt{data\_object\_references} & 15 & 3958 \\
\texttt{data\_association\_references} & 12 & 25391 \\
\texttt{data\_association\_relationships} & 13 & 1422 \\
\texttt{data\_companion\_separations} & 21 & 210 \\
\texttt{data\_astro\_sequences} & 15 & 30676 \\
\texttt{data\_spectra} & 8 & 26636194 \\
\texttt{data\_relative\_radial\_velocities\_std} & 25 & 754 \\
\texttt{data\_mamajek\_table} & 34 & 124 \\
\texttt{data\_teff} & 33 & 8731800 \\
\texttt{data\_spectral\_types} & 52 & 4438488 \\
\texttt{data\_spectral\_types\_field\_ucds} & 47 & NaN \\
\texttt{data\_radial\_velocities} & 30 & 1276996 \\
\texttt{data\_relative\_radial\_velocities} & 26 & 64480 \\
\texttt{data\_vsini} & 31 & 275101 \\
\texttt{data\_equivalent\_widths} & 33 & 106953 \\
\texttt{calc\_banyan\_sigma\_best} & 43 & NaN \\
\texttt{calc\_equivalent\_widths\_combined} & 23 & 14558 \\
\texttt{calc\_radial\_velocities\_combined} & 24 & 553854 \\
\texttt{calc\_spectral\_indices\_combined} & 23 & 22413 \\
\texttt{calc\_ecliptic\_coordinates} & 9 & NaN \\
\texttt{calc\_radial\_velocities\_corrected} & 27 & 1383947 \\
\texttt{calc\_banyan\_sigma\_details} & 26 & 45576696 \\
\texttt{calc\_object\_age\_pdfs} & 5 & 630989312 \\
\texttt{calc\_association\_age\_pdfs} & 5 & 53759812 \\
\texttt{calc\_vsini\_predictions} & 21 & 72717 \\
\texttt{calc\_comover\_probability} & 52 & 9328 \\
\texttt{calc\_banyan\_sigma\_model\_properties} & 81 & 19367 \\
\texttt{calc\_uvw\_raw} & 37 & 559758 \\
\texttt{calc\_banyan\_sigma} & 48 & 39756309 \\
\texttt{calc\_uvw} & 47 & 1156536 \\
\texttt{calc\_vtan} & 10 & NaN \\
\texttt{calc\_xyz} & 25 & 3169606 \\
\texttt{mechanics\_memberships\_aggregated} & 5 & 5525665 \\
\texttt{mechanics\_object\_properties\_combined} & 14 & 128170 \\
\texttt{mechanics\_all\_designations} & 13 & 22497442 \\
\texttt{mechanics\_association\_designations} & 12 & 35688 \\
\texttt{mechanics\_files} & 13 & 125789 \\
\texttt{mechanics\_banyan\_sigma\_model\_inputs} & 65 & 13400268 \\
\texttt{mechanics\_combinatory\_logic} & 11 & 34 \\
\texttt{mechanics\_automatically\_rejected\_memberships} & 11 & 154607 \\
\texttt{mechanics\_gaiadr3\_neighborhood} & 15 & 1049413 \\
\texttt{mechanics\_memberships\_propagated} & 18 & 4513706 \\
\texttt{mechanics\_all\_association\_relationships} & 9 & 2949 \\
\texttt{mechanics\_file\_sets} & 11 & 101362 \\
\texttt{mechanics\_memberships\_vetted} & 18 & 4485047 \\
\texttt{mechanics\_object\_xmatch} & 23 & 11341867 \\
\texttt{summary\_all\_members\_both} & 32 & 7444747 \\
\texttt{summary\_white\_dwarfs} & 18 & NaN \\
\texttt{summary\_giants} & 18 & NaN \\
\texttt{summary\_all\_members} & 31 & NaN \\
\texttt{summary\_all\_objects} & 12 & NaN \\
\texttt{summary\_planemos} & 13 & NaN \\
\texttt{summary\_all\_members\_both\_veryold} & 29 & 5713768 \\
\enddata
\end{deluxetable*}


==> tables/rej_planemos.tex <==
\clearpage
\pagebreak
{
\ifpdf
\pdfpageattr{/Rotate 90}
\fi
\movetabledown=70mm
\begin{rotatetable*}
\begin{deluxetable*}{lcclcllcccl}
\tablewidth{0.985\textwidth}
\tablecaption{Literature Planetary-Mass Objects which Membership is not Corroborated by BANYAN~$\Sigma$.\label{tab:rej_planemos}}
\tablehead{
\noalign{\vskip 1.0ex}
\colhead{Designation} & \colhead{\shortstack{Spectral\\ Type}} & \colhead{\shortstack{Banyan~$\Sigma$\\ $P$ (\%)}} & \colhead{\shortstack{Lit.\\ Memberships}} & \colhead{\shortstack{Distance\\ (pc)}} & \colhead{\shortstack{Right\\ Ascension}} & \colhead{Decl.} & \colhead{\shortstack{$\mu_\alpha\cos\delta$\\ (\masyr)}} & \colhead{\shortstack{$\mu_\delta$\\ (\masyr)}} & \colhead{\shortstack{RV\\(\kms)}} & \colhead{Refs\tablenotemark{a}}
}
\startdata
$[$AKC2006$]$ 17 & L0 & 1.2 & LUP,CM & $305 \pm 99$ & 15:39:27.25 & -34:48:44.1 & $-12 \pm 2$ & $-4 \pm 1$ & $\cdots$ & 1;2;--;2;3 \\
2MASS J00464841+0715177 & L0$\delta$ & 0.0 & BPMG,CM & $37.8 \pm 0.4$ & 00:46:48.42 & 07:15:17.7 & $95.5 \pm 0.3$ & $-60.3 \pm 0.3$ & $-2.8 \pm 0.3$ & 4;2;--;2;4 \\
2MASS J01531463-6744181 & L3$\beta$ & 2.2 & THA,CM & $(25 \pm 5)$ & 01:53:14.63 & -67:44:18.2 & $82 \pm 3$ & $-21 \pm 9$ & $\cdots$ & 4;5;--;6;4 \\
2MASS J02411151-0326587 & L0$\gamma$ & 1.2 & THA,CM & $56 \pm 7$ & 02:41:11.52 & -03:26:58.8 & $69.6 \pm 0.5$ & $-25.1 \pm 0.6$ & $6 \pm 8$ & 7;8;--;8;4 \\
2MASS J04215450+2652315 & M8.5 & 4.9 & TAU,CM & $\cdots$ & 04:21:54.53 & 26:52:31.4 & $12 \pm 4$ & $-9 \pm 4$ & $\cdots$ & 9;10;--;--;11 \\
2MASS J04311907+2335047 & M7.75 & 4.6 & TAU,HM & $168 \pm 8$ & 04:31:19.08 & 23:35:04.5 & $7.7 \pm 0.3$ & $-16.1 \pm 0.3$ & $32.3 \pm 0.6$ & 9;2;--;2;12 \\
2MASS J04373705+2331080 & L0 & 5.1 & TAU,CM & $(31 \pm 7)$ & 04:37:37.05 & 23:31:08.1 & $4 \pm 3$ & $-19 \pm 3$ & $\cdots$ & 9;13;--;6;14 \\
2MASS J06085283-2753583 & L0 $\delta$ & 10.0 & COL,LM & $44.2 \pm 0.3$ & 06:08:52.85 & -27:53:58.2 & $12.4 \pm 0.2$ & $6.2 \pm 0.2$ & $26.7 \pm 0.6$ & 4;2;--;2;4 \\
2MASS J09553336-0208403 & L7pec(red) & 0.0 & TWA,CM & $(29 \pm 6)$ & 09:55:33.36 & -02:08:40.4 & $-117 \pm 2$ & $-94 \pm 2$ & $-20 \pm 4$ & 15;16;--;6;15 \\
2MASS J10212570-2830427 & L5$\beta$ & 0.0 & TWA,CM & $(10 \pm 2)$ & 10:21:25.71 & -28:30:42.8 & $-49 \pm 8$ & $-56 \pm 6$ & $\cdots$ & 15;17;--;6;4 \\
2MASS J11472421-2040204 & L7pec(red) & 6.0 & TWA,CM & $38 \pm 3$ & 11:47:24.21 & -20:40:20.4 & $-118 \pm 2$ & $-71 \pm 3$ & $7 \pm 3$ & 15;18;--;18;19 \\
2MASS J12271545-0636458 & M8.5$\beta$ & 0.1 & TWA,CM & $39.1 \pm 0.5$ & 12:27:15.32 & -06:36:46.9 & $-120.2 \pm 0.3$ & $-53.9 \pm 0.2$ & $\cdots$ & 4;2;--;2;4 \\
2MASS J12563961-2718455 & L4$\beta$ & 2.5 & TWA,CM & $(32 \pm 8)$ & 12:56:39.61 & -27:18:45.6 & $-77 \pm 8$ & $-66 \pm 4$ & $-19 \pm 4$ & 15;20;--;6;4 \\
2MASS J16072342-3905099 & L1 & 0.0 & LUPIII,CM & $3,161 \pm 1,628$ & 16:07:23.41 & -39:05:09.9 & $-4.3 \pm 0.4$ & $-1.3 \pm 0.3$ & $\cdots$ & 21;2;--;2;21 \\
2MASS J16262218-2423523 & M8.5 & 0.0 & ROPH,CM & $\cdots$ & 16:26:22.19 & -24:23:52.4 & $2 \pm 2$ & $-1 \pm 2$ & $\cdots$ & --;16;--;--;22 \\
2MASS J16263252-2426354 & M8 & 0.0 & ROPH,CM & $\cdots$ & 16:26:32.52 & -24:26:35.4 & $9 \pm 2$ & $1 \pm 2$ & $\cdots$ & --;16;--;--;22 \\
2MASS J16263991-2422334 & M8.3 & 0.0 & ROPH,CM & $\cdots$ & 16:26:39.92 & -24:22:33.4 & $-0 \pm 2$ & $2 \pm 2$ & $\cdots$ & 23;16;--;--;22 \\
2MASS J16270592-2418402 & L3 & 5.1 & ROPH,CM & $(22 \pm 4)$ & 16:27:05.93 & -24:18:40.2 & $-3 \pm 2$ & $-18 \pm 2$ & $\cdots$ & 24;16;--;6;22 \\
2MASS J19350976-6200473 & L1$\gamma$ & 2.7 & THA,CM & $(31 \pm 7)$ & 19:35:09.77 & -62:00:47.3 & $-3 \pm 8$ & $-102 \pm 7$ & $\cdots$ & 4;25;--;6;4 \\
2MASS J20113196-5048112 & L3$\gamma$ & 9.2 & THA,CM & $2,042 \pm 1,315$ & 20:11:31.96 & -50:48:11.2 & $23 \pm 3$ & $-77 \pm 3$ & $\cdots$ & 4;17;--;2;4 \\
2MASS J22134491-2136079 & L0$\gamma$ & 0.0 & BPMG,LM & $48 \pm 2$ & 22:13:44.92 & -21:36:08.0 & $52.3 \pm 0.8$ & $-73.8 \pm 0.9$ & $-5 \pm 4$ & 7;2;--;2;4 \\
2MASS J22163082+1953167 & T3 & 0.0 & BPMG,CM & $1,495 \pm 569$ & 22:16:30.83 & 19:53:16.7 & $-0.3 \pm 0.2$ & $0.1 \pm 0.3$ & $\cdots$ & 26;2;--;2;26 \\
2MASS J22351658-3844154 & L1.5$\gamma$ & 0.0 & THA,CM & $41 \pm 2$ & 22:35:16.59 & -38:44:15.4 & $60.1 \pm 0.8$ & $-84 \pm 1$ & $\cdots$ & 4;2;--;2;4 \\
2MASS J22353560-5906306 & M8.5 & 5.6 & THA,CM & $46.9 \pm 0.5$ & 22:35:35.61 & -59:06:30.6 & $60.4 \pm 0.2$ & $-84.2 \pm 0.2$ & $\cdots$ & 27;2;--;2;4 \\
2MASS J13005303-7709478 & M9 & 0.1 & CHAII,CM & $\cdots$ & 13:00:53.030 & -77:09:47.90 & $-26 \pm 1$ & $-3 \pm 1$ & $\cdots$ & 28;17;--;--;28 \\
2MASS J16144169-2351058 & L1 & 2.3 & USCO,HM & $(30 \pm 8)$ & 16:14:41.696 & -23:51:05.82 & $-7 \pm 1$ & $-14 \pm 1$ & $\cdots$ & 29;16;--;6;30 \\
UGCS J160420.42-213452.9 & L2 & 0.1 & USCO,CM & $(74 \pm 21)$ & 16:04:20.420 & -21:34:53.00 & $-2 \pm 6$ & $15 \pm 6$ & $\cdots$ & 31;17;--;6;32 \\
MOCA J160731618-21465440 & L1 & 0.0 & USCO,HM & $992 \pm 974$ & 16:07:31.618 & -21:46:54.40 & $-2 \pm 2$ & $-6 \pm 1$ & $\cdots$ & 31;2;--;2;31 \\
UGCS J160843.43-224516.0 & L1 & 0.7 & USCO,HM & $580 \pm 534$ & 16:08:43.435 & -22:45:16.12 & $12 \pm 1$ & $-8 \pm 1$ & $\cdots$ & 31;2;--;2;30 \\
UGCS J161512.69-222949.1 & L4 & 4.5 & USCO,CM & $(63 \pm 16)$ & 16:15:12.700 & -22:29:49.20 & $41 \pm 18$ & $4 \pm 18$ & $\cdots$ & 31;16;--;6;32 \\
2MASS J04210636+2706545 & M9.5 & 2.2 & TAU,CM & $\cdots$ & 04:21:06.364 & +27:06:54.57 & $14 \pm 14$ & $-14 \pm 14$ & $\cdots$ & 9;25;--;--;33 \\
2MASS J04220204+1947499 & M9 & 0.4 & TAU,CM & $\cdots$ & 04:22:02.047 & +19:47:49.00 & $-1 \pm 4$ & $-5 \pm 4$ & $\cdots$ & 9;13;--;--;33 \\
2MASS J04282999+2358482 & M9.25 & 0.5 & TAU,CM & $\cdots$ & 04:28:30.011 & +23:58:48.08 & $6 \pm 2$ & $-11 \pm 2$ & $\cdots$ & 9;13;--;--;33 \\
UGCS J043328.48+175833.0 & L0 & 6.6 & TAU,CM & $(52 \pm 10)$ & 04:33:28.477 & +17:58:33.05 & $12 \pm 3$ & $-11 \pm 3$ & $\cdots$ & 9;13;--;6;33 \\
UGCS J043506.95+230750.7 & L0 & 0.0 & TAU,CM & $1,057 \pm 41$ & 04:35:06.953 & +23:07:50.69 & $10.47 \pm 0.05$ & $-4.57 \pm 0.03$ & $\cdots$ & 9;2;--;2;33 \\
2MASS J03442789+3227189 & M6 & 0.2 & IC348,HM & $\cdots$ & 03:44:27.895 & +32:27:18.78 & $7 \pm 2$ & $-8 \pm 2$ & $16.5 \pm 1.0$ & 34;6;--;--;35 \\
2MASS J11080609-7739406 & M9 & 0.2 & CHAI,HM & $\cdots$ & 11:08:06.093 & -77:39:40.68 & $-24 \pm 2$ & $5 \pm 2$ & $\cdots$ & 36;17;--;--;36 \\
2MASS J11084952-7638443 & M8.8 & 0.1 & CHAI,HM & $\cdots$ & 11:08:49.398 & -76:38:44.26 & $-24.0 \pm 0.8$ & $6 \pm 1$ & $\cdots$ & 36;6;--;--;36 \\
2MASS J11100658-7642486 & M9.3 & 0.1 & CHAI,HM & $\cdots$ & 11:10:06.588 & -76:42:48.66 & $-21.9 \pm 0.6$ & $2.7 \pm 0.7$ & $\cdots$ & 36;6;--;--;36 \\
2MASS J15451990-2616529 & M8-L0 & 2.9 & USCO,CM & $\cdots$ & 15:45:19.910 & -26:16:52.97 & $-17 \pm 3$ & $-24 \pm 3$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J15473372-2447475 & M9 & 0.2 & USCO,CM & $\cdots$ & 15:47:33.726 & -24:47:47.55 & $-17 \pm 2$ & $-20 \pm 2$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J15550979-2313266 & M9.5 & 7.8 & USCO,CM & $\cdots$ & 15:55:09.798 & -23:13:26.62 & $-12.0 \pm 0.9$ & $-23.0 \pm 0.8$ & $\cdots$ & 37;6;--;--;31 \\
2MASS J15562344-2541056 & L0.5 & 0.0 & USCO,CM & $(35 \pm 11)$ & 15:56:23.449 & -25:41:05.61 & $-18.32 \pm 0.03$ & $-22.48 \pm 0.02$ & $-0.89 \pm 0.02$ & 38;2;--;6;31 \\
2MASS J16013934-2447098 & M8.5: & 1.7 & USCO,CM & $\cdots$ & 16:01:39.317 & -24:47:10.37 & $-13 \pm 2$ & $-23 \pm 2$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16064555-2121589 & M9.5 & 2.9 & USCO,CM & $\cdots$ & 16:06:45.552 & -21:21:58.91 & $-16 \pm 3$ & $-26 \pm 3$ & $\cdots$ & 37;17;--;--;32 \\
2MASS J16115691-1906466 & M9 & 8.8 & USCO,CM & $\cdots$ & 16:11:56.912 & -19:06:46.64 & $-9 \pm 6$ & $-21 \pm 6$ & $\cdots$ & 37;17;--;--;31 \\
2MASS J16142929-2417404 & M8 & 0.0 & USCO,CM & $\cdots$ & 16:14:29.291 & -24:17:40.95 & $-14 \pm 1$ & $-20 \pm 1$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16173081-2411411 & M9 & 0.8 & USCO,CM & $\cdots$ & 16:17:30.814 & -24:11:41.19 & $-14.4 \pm 0.5$ & $-28.0 \pm 0.6$ & $\cdots$ & 37;6;--;--;31 \\
2MASS J16173147-2404164 & M8-L0 & 0.7 & USCO,CM & $\cdots$ & 16:17:31.475 & -24:04:16.92 & $-7 \pm 1$ & $-19 \pm 1$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16183182-2253149 & M8-L0 & 7.0 & USCO,CM & $\cdots$ & 16:18:31.809 & -22:53:15.59 & $-8 \pm 4$ & $-22 \pm 4$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16183770-2303080 & M9 & 2.1 & USCO,CM & $\cdots$ & 16:18:37.695 & -23:03:08.53 & $-4 \pm 2$ & $-16 \pm 2$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16193507-2327252 & M9.5 & 0.8 & USCO,CM & $\cdots$ & 16:19:35.051 & -23:27:25.76 & $-5 \pm 1$ & $-17 \pm 1$ & $\cdots$ & 37;16;--;--;31 \\
2MASS J16203052-2144503 & M8.5 & 1.1 & USCO,CM & $\cdots$ & 16:20:30.529 & -21:44:50.33 & $-8.1 \pm 0.9$ & $-20.7 \pm 0.9$ & $\cdots$ & 37;6;--;--;31 \\
BKLT J162736-245134 & L0 & 9.5 & ROPH,CM & $(26 \pm 5)$ & 16:27:36.612 & -24:51:36.09 & $-8 \pm 2$ & $-21 \pm 2$ & $\cdots$ & 24;16;--;6;39 \\
BKLT J162810-242421 & L0 & 5.4 & ROPH,CM & $(31 \pm 6)$ & 16:28:10.451 & -24:24:20.07 & $-4 \pm 2$ & $-19 \pm 2$ & $\cdots$ & 24;16;--;6;39 \\
CFHTWIR-Oph 18 & L0 & 0.0 & ROPH,CM & $(339 \pm 86)$ & 16:26:19.409 & -24:27:43.80 & $1 \pm 3$ & $1 \pm 3$ & $\cdots$ & 24;16;--;6;39 \\
CFHTWIR-Oph 77 & M9.8 & 0.3 & ROPH,CM & $\cdots$ & 16:27:25.644 & -24:37:28.52 & $-12 \pm 21$ & $-18 \pm 22$ & $\cdots$ & 24;25;--;--;39 \\
NAME Cha J1305-7739 & L1 & 0.4 & CHAII,HM & $(46 \pm 9)$ & 13:05:40.800 & -77:39:58.20 & $-21 \pm 6$ & $-2 \pm 7$ & $\cdots$ & 40;17;--;6;41 \\
OTS 44 & M9.5 & 0.3 & CHAI,HM & $\cdots$ & 11:10:09.344 & -76:32:17.85 & $-23 \pm 2$ & $1 \pm 2$ & $\cdots$ & 36;17;--;--;42 \\
$\[$L2007b$\]$ Cha J11105772-7714570 & M9.5 & 0.2 & CHAI,HM & $\cdots$ & 11:10:57.720 & -77:14:57.00 & $-22 \pm 3$ & $2 \pm 3$ & $\cdots$ & 43;17;--;--;43 \\
CFBDSIR J214947.2-040308.9 & T7.5 (red) & 0.0 & ABDMG,CM & $56 \pm 6$ & 21:49:47.20 & -04:03:08.9 & $138 \pm 1$ & $-94 \pm 2$ & $8 \pm 4$ & 44;44;--;44;45 \\
SDSS J121951.45+312849.4 & L8 & 0.4 & ARG,BF & $20 \pm 2$ & 12:19:51.528 & +31:28:49.44 & $-248 \pm 2$ & $-21 \pm 4$ & $-19 \pm 4$ & 46;20;--;18;47 \\
CWISE J041953.55+203628.0 & T4 & 0.0 & HYA,CM & $2,803 \pm 1,273$ & 04:19:53.554 & +20:36:28.04 & $0.3 \pm 0.3$ & $0.1 \pm 0.3$ & $\cdots$ & 48;2;--;2;48 \\
\enddata
\tablenotetext{a}{References for spectral types, proper motions, radial velocities, distances, and memberships, respectively.}
\tablecomments{Distances between parentheses are photometric rather than trigonometric.}
\tablerefs{(1)~\cite{2006ApJ...647L.167J}, (2)~\cite{2023AA...674A...1G}, (3)~\cite{2008ApJS..177..551M}, (4)~\cite{2015ApJS..219...33G}, (5)~\cite{2015ApJ...798...73G}, (6)~This Paper, (7)~\cite{2009AJ....137.3345C}, (8)~\cite{2016ApJ...833...96L}, (9)~\cite{2023AJ....165...37L}, (10)~\cite{2018ApJ...858...41Z}, (11)~\cite{2009ApJ...703..399L}, (12)~\cite{2006AJ....132.2665S}, (13)~\cite{2025AJ....170...86S}, (14)~\cite{2017ApJ...837...95B}, (15)~\cite{2017ApJS..228...18G}, (16)~\cite{2007MNRAS.379.1599L}, (17)~\cite{2021AJ....161..192N}, (18)~\cite{2020AJ....159..257B}, (19)~\cite{2016ApJ...822L...1S}, (20)~\cite{2018ApJS..234....1B}, (21)~\cite{2005AA...440..139L}, (22)~\cite{2008hsf2.book..351W}, (23)~\cite{2011ApJ...726...23G}, (24)~\cite{2012AA...539A.151A}, (25)~\cite{2021ApJS..253....8M}, (26)~\cite{2015ApJ...814..118B}, (27)~\cite{2024AJ....168..159L}, (28)~\cite{2008ApJ...680.1295S}, (29)~\cite{2011AA...527A..24L}, (30)~\cite{2007MNRAS.374..372L}, (31)~\cite{2018AJ....156...76L}, (32)~\cite{2013MNRAS.435.2474L}, (33)~\cite{2019AJ....158...54E}, (34)~\cite{2023ApJS..267....7Z}, (35)~\cite{2018ApJ...869...72Y}, (36)~\cite{2007ApJS..173..104L}, (37)~\cite{2020AJ....160...44L}, (38)~\cite{2020AA...633A.152C}, (39)~\cite{2010AA...515A..75A}, (40)~\cite{2007ApJ...657..511A}, (41)~\cite{2008ApJ...676..427A}, (42)~\cite{2007ApJ...662..413K}, (43)~\cite{2017AJ....154...46E}, (44)~\cite{2017AA...602A..82D}, (45)~\cite{2012AA...548A..26D}, (46)~\cite{2006AJ....131.2722C}, (47)~\cite{Best20US}, (48)~\cite{2022AJ....163..242S}.}
\end{deluxetable*}
\end{rotatetable*}
}

